Monocular Depth Estimators: Vulnerabilities and Attacks

Recent advancements of neural networks lead to reliable monocular depth estimation. Monocular depth estimated techniques have the upper hand over traditional depth estimation techniques as it only needs one image during inference. Depth estimation is one of the essential tasks in robotics, and monocular depth estimation has a wide variety of safety-critical applications like in self-driving cars and surgical devices. Thus, the robustness of such techniques is very crucial. It has been shown in recent works that these deep neural networks are highly vulnerable to adversarial samples for tasks like classification, detection and segmentation. These adversarial samples can completely ruin the output of the system, making their credibility in real-time deployment questionable. In this paper, we investigate the robustness of the most state-of-the-art monocular depth estimation networks against adversarial attacks. Our experiments show that tiny perturbations on an image that are invisible to the naked eye (perturbation attack) and corruption less than about 1% of an image (patch attack) can affect the depth estimation drastically. We introduce a novel deep feature annihilation loss that corrupts the hidden feature space representation forcing the decoder of the network to output poor depth maps. The white-box and black-box test compliments the effectiveness of the proposed attack. We also perform adversarial example transferability tests, mainly cross-data transferability.

==> tables/blackbox_patch_rmse.tex <==
%\begin{table*}
	\begin{tabular}{l|c|c|c}
		\hline
		Methods & Clean & \multicolumn{2}{c}{Attacked} \\
		\cline{2-4}
		& RMSE         & RMSE   & Rel (\%)   \\
		\hline
		SFM      & 6.1711       & 7.5363      & 23    \\
		B2F      & 5.1615       & 5.6992     & 11    \\
		SCSFM    & 5.2271       & 6.5846     & 26    \\
		Mono1    & 5.1973       & 5.9163     & 14     \\
		Mono2    & 4.9099       & 5.4289     & 11    \\
		\hline
	\end{tabular}
%	\caption{Black-box Patch Attack $72 \times 72$. RMSE.}
%	\label{blackbox_patch_rmse}
%\end{table*}

==> tables/blackbox_pert_rmse.tex <==
%\begin{table*}
	\begin{tabular}{l|c|c|c}
		\hline
		Methods & Clean & \multicolumn{2}{c}{Attacked} \\
		\cline{2-4}
		& RMSE         & RMSE   & Rel (\%)   \\
		\hline
		SFM      & 6.1711       & 6.816      & 11    \\
		B2F      & 5.1615       & 5.9961     & 17    \\
		SCSFM    & 5.2271       & 5.7216     & 10    \\
		Mono1    & 5.1973       & 5.5388     & 7     \\
		Mono2    & 4.9099       & 5.7408     & 17    \\
		\hline
	\end{tabular}
%	\caption{Black-box Perturbation Attack $\eta=0.05$. RMSE.}
%	\label{blackbox_pert_rmse}
%\end{table*}
